Leveraging Flatness to Improve Information-Theoretic Generalization Bounds for SGD

Information-theoretic (IT) generalization bounds have been used to study the generalization of learning algorithms. These bounds are intrinsically data- and algorithm-dependent so that one can exploit the properties of data and algorithm to derive tighter bounds. However, we observe that although the flatness bias is crucial for SGD's generalization, these bounds fail to capture the improved generalization under better flatness and are also numerically loose. This is caused by the inadequate leverage of SGD's flatness bias in existing IT bounds. This paper derives a more flatness-leveraging IT bound for the flatness-favoring SGD. The bound indicates the learned models generalize better if the large-variance directions of the final weight covariance have small local curvatures in the loss landscape. Experiments on deep neural networks show our bound not only correctly reflects the better generalization when flatness is improved, but is also numerically much tighter. This is achieved by a flexible technique called "omniscient trajectory". When applied to Gradient Descent's minimax excess risk on convex-Lipschitz-Bounded problems, it improves representative IT bounds' $\Omega(1)$ rates to $O(1/\sqrt{n})$. It also implies a by-pass of memorization-generalization trade-offs.

==> algorithm/algo.tex <==
\input{theory/extra.tex}

==> theory/extra.tex <==
\begin{theorem}\label{theorem:negrea}
    
\end{theorem}

==> theory/minimax/negative.tex <==
\subsection{Proof of \cref{prop:minimax_negative}}

\begin{proposition}\label{prop:minimax_negative}
    \begin{multline}
        \gen[\mu^n][\GDalgo] \\
        \le \inf_{\prob{\Delta G}} \frac{L D}{n} \sum_{i=1}^n \sqrt{8 I(W_T + \Delta G; U_i \mid \tilde{S}, U_{-i})} +  \ex{\absDelta_{\weights, \Delta G}(\weight_T, \trainingSet)} + \ex{\absDelta_{\weights, \Delta G}(\weight_T, \trainingSet')} \\ = \Omega(1),
    \end{multline}
    where
    \begin{align}
        \absDelta_{\weights, \Delta g}(\instanceWeight, \instanceTrainingSet) \defeq \opabs{
            \emploss[\instanceTrainingSet]{\proj(\instanceWeight + \Delta g)} - \emploss[\instanceTrainingSet]{\instanceWeight}
        }
    \end{align}


\end{proposition}

\TODO{}

\begin{lemma}[Extended from Lemma 2 of \citet{livni2024information}]\label{lemma:MI_and_correlation}
    Let $X, Y \in \reals^d$ be two random variables such that $\norm{X} \le r$, $\ex{X} = 0$ and $\ex{\norm{Y}^2} \le v^2 \le 2$. If $\ex{X^\top Y} = \beta$, then
    \begin{align}
        \sqrt{I(X; Y)} \ge \frac{2-v^2}{2 \sqrt{2} r^2} \beta^2.
    \end{align}
\end{lemma}

\begin{proof}
    The proof is adapted from Lemma 2 of \citet{livni2024information} with the following differences: 1) to handle the infinite domain of the random variables, we replace the combo of total variation and the coupling lemma with 2-Wasserstein distances and the couplings provided by it, resembled from \citet{haghifam_limitations_2023}'s Theorem 11; and 2) we allow random variables to have many dimensions, which is a minor extension.

    \NewDocumentCommand{\convenientWass}{O{Y}}{\wass{\prob{X}}{\prob{X\mid #1}}}
    \NewDocumentCommand{\virtualX}{}{\bar{X}}
    \NewDocumentCommand{\virtualY}{}{\bar{Y}}
    \NewDocumentCommand{\virtualCoupledX}{}{\virtualX_{\virtualY}}

    Let $\prob{X, Y}$ be the joint distribution of the RVs.
    Let $\wass{\cdot}{\cdot}$ be the 2-Wasserstein distance defined by
    \begin{align}
        \wass{\prob{A}}{\prob{B}} \defeq \inf_{Q_{\bar{A}, \bar{B}}: Q_{\bar{A}} = \prob{A}, Q_{\bar{B}} = \prob{B}} \ex{\norm{\bar{A} - \bar{B}}^2},
    \end{align}
    According to Theorem 6.15 of \citet{villani2009optimal} that exploits the boundedness of $X$ and the Pinsker's inequality \citep{golden_formula}, we have given any $y$,
    \begin{align}
        \wass{\prob{X}}{\prob{X \mid y}}
        \unimportant{
        \le&    \wass[2]{\prob{X}}{\prob{X \mid y}}^2\\
        \le&    \left(2^{1/2} \left(\int d(x_0, x)^2 d|\mu-\nu|(x)\right)^{1/2}\right)^2\\
        =&  2 \left(\int d(0, x)^2 d|\mu - \nu|(x)\right)\\
        \le& 2 \left(\int r^2 d|\mu - \nu|(x)\right)\\
        =& 2 r^2 \left(\int d|\mu - \nu|(x)\right)\\
        }
        \le&    2 r^2 \tv{\prob{X}}{\prob{X \mid y}} 
        \le     2 r^2 \sqrt{2 \kl{\prob{X}}{\prob{X \mid y}}}.
    \end{align}
    Taking expectation over $y$ and by the concavity of the square root, we have
    \begin{align}
        \ex[Y]{\wass{\prob{X}}{\prob{X \mid y}}}
        \le&     \ex[Y]{2 r^2 \sqrt{2\kl{\prob{X}}{\prob{X \mid Y}}}}
        \le 2 r^2 \sqrt{2 \ex[Y]{\kl{\prob{X}}{\prob{X \mid Y}}}}\\
        =&  2 r^2 \sqrt{2 I(X; Y)}.
    \end{align}
    

    \NewDocumentCommand{\convenientCoupling}{O{Y}}{\coupling{\virtualX, \virtualX_{#1}}[\epsilon, #1]}
    \NewDocumentCommand{\convenientJoint}{O{Y} O{Y, \virtualX, \virtualX_{#1}}}{\coupling{#2}[\epsilon]}
    We then relate the Wasserstein distance to the correlation between $X$ and $Y$.
    By definition of the Wasserstein distance, given $y$, for any $\epsilon > 0$, we have an ($(\epsilon, y)$-dependent) coupling $\convenientCoupling[y]$ over $\reals^d \times \reals^d$  such that $Q^{\epsilon, y}_{\virtualX} = \prob{X}$, $Q^{\epsilon, y}_{\virtualX_y} = \prob{X \mid y}$, and
    \begin{align}
        \convenientWass[y] \le \ex[\convenientCoupling[y]]{\norm{\virtualX - \virtualX_y}^2} \le \convenientWass[y] + \epsilon. \label{eq:wass_coupling}
    \end{align}
    Fix an $\epsilon > 0$. Consider the following random process: $\virtualY \to (\virtualX, \virtualCoupledX)$, where one first sample $\virtualY \sim \prob{Y}$, and then sample $(\virtualX, \virtualCoupledX) \sim \convenientCoupling$. Denote the joint distribution of the process by $\convenientJoint$. 
    By \cref{eq:wass_coupling}, we have
    \begin{align}
        \ex[Y]{\convenientWass[Y]} \le \ex[\convenientJoint[Y]]{\norm{\virtualX - \virtualCoupledX}^2} \le \ex[Y]{\convenientWass[Y]} + \epsilon, 
    \end{align}
    and
    \begin{align}
        \sqrt{I(X; Y)} \ge \frac{1}{2 \sqrt{2} r^2} \left(\ex{\norm{\virtualX - \virtualCoupledX}^2} - \epsilon\right). \label{eq:MI_and_correlated-uncorrelated_difference}
    \end{align}
    
    Now we lower-bound the above squared distance between the $\virtualY$-uncorrelated $\virtualX$ and the $\virtualY$-correlated $\virtualCoupledX$ using the correlation between $X$ and $Y$.
    \begin{align}
        \ex[\convenientJoint[Y]]{\norm{\virtualX - \virtualCoupledX}^2}
        =&  \ex{\norm{\virtualX}^2} + \ex{\norm{\virtualCoupledX}^2} - 2\ex{\virtualX^\top \virtualCoupledX}
        =   2 \ex{\norm{X}^2} - 2 \ex{\virtualX^\top \virtualCoupledX}. \label{eq:correlated-uncorrelated_difference}
    \end{align}
    To capture the correlated part of $\virtualCoupledX$ with $\virtualY$, as \citet{livni2024information}, we rewrite $\virtualCoupledX$ as $\beta \virtualY$ and the residual by $\virtualCoupledX = \beta \virtualY + (\virtualCoupledX - \beta \virtualY)$, which leads to
    \begin{align}
        \ex{\virtualX^\top \virtualCoupledX}
        =&  \beta \ex{\virtualX^\top \virtualY} + \ex{\virtualX^\top (\virtualCoupledX - \beta \virtualY)}. 
    \end{align}
    Since $\convenientJoint[][\virtualX \mid y] = Q^{\epsilon, y}_{\virtualX} = \prob{X}$ regardless of $y$, $\virtualX$ is independent with $\virtualY$, and we have
    \begin{align}
        \ex{\virtualX^\top \virtualY} = \ex{\virtualX}^\top \ex{\virtualY} = 0.
    \end{align}
    Applying this and using the Cauchy-Schwarz inequality lead to
    \begin{align}
        \ex{\virtualX^\top \virtualCoupledX}
        =&  \ex{\virtualX^\top (\virtualCoupledX - \beta \virtualY)} 
        \unimportant{
        =&  \sqrt{\ex{\virtualX^\top (\virtualCoupledX - \beta \virtualY)}^2}\\
        }
        \le   \sqrt{\ex{\norm{\virtualX}^2} \ex{\norm{\virtualCoupledX - \beta \virtualY}^2}}. \label{eq:correlated-uncorrelated_product}
    \end{align}

    Since $\convenientJoint[][\virtualY, \virtualCoupledX] = \prob{Y, X}$, we have
    \begin{align}
        \ex{\virtualCoupledX^\top \virtualY} = \ex{X^\top Y} = \beta,
    \end{align}
    and applying this leads to
    \begin{align}
        \ex{\norm{\virtualCoupledX - \beta \virtualY}^2}
        =&  \ex{\norm{\virtualCoupledX}^2} + \beta^2 \ex{\norm{\virtualY}^2} - 2 \beta \ex{\virtualCoupledX^\top \virtualY}\\
        \le&    \ex{\norm{X}^2} + v^2 \beta^2 - 2 \beta^2 = \ex{\norm{X}^2} - (2 - v^2)\beta^2. \label{eq:residual_norm}
    \end{align}
    
    Plugging \cref{eq:correlated-uncorrelated_difference,eq:correlated-uncorrelated_product,eq:residual_norm} leads to
    \begin{align}
        & \ex{\norm{\virtualX - \virtualCoupledX}^2}\\
        \ge&  2 \ex{\norm{X}^2} - 2 \sqrt{\ex{\norm{X}^2}(\ex{\norm{X}^2} - (2-v^2)\beta^2)}\\
        =&  2 \sqrt{\ex{\norm{X}^2}} \left(\sqrt{\ex{\norm{X}^2}} - \sqrt{\ex{\norm{X}^2} - (2-v^2)\beta^2}\right)\\
        &(\text{$2-v^2 >= 0$})\\
        \ge&    \left(\sqrt{\ex{\norm{X}^2}} + \sqrt{\ex{\norm{X}^2} - (2-v^2)\beta^2}\right) \left(\sqrt{\ex{\norm{X}^2}} - \sqrt{\ex{\norm{X}^2} - (2-v^2)\beta^2}\right)\\
        =&  (2-v^2) \beta^2.
    \end{align}
    Combining \cref{eq:MI_and_correlated-uncorrelated_difference}, we have
    \begin{align}
        \sqrt{I(X; Y)} \ge \frac{1}{2 \sqrt{2} r^2} \left((2 - v^2) \beta^2 - \epsilon\right).
    \end{align}
    By arbitrariness of $\epsilon > 0$, we have
    \begin{align}
        \sqrt{I(X; Y)} \ge \frac{2 - v^2}{2 \sqrt{2} r^2} \beta^2.
    \end{align}
\end{proof}

\NewDocumentCommand{\pmBernoulli}{m}{B_{#1}}

For any $p \in [-1, +1]$, let $\pmBernoulli{p}$ denote the distribution over $\set{-1, +1}$ such that the expectation is $p$.

\begin{lemma}[Extended from Lemma A.1 of \citet{bun_make_2017}]\label{lemma:expectation_and_derivative}
    Let $\tilde{f}$ be a \emph{stochastic} mapping from $\set{\pm 1}^{n} \times [-1, +1]$ to $\reals$ such that its expectation $\ex{\tilde{f}(X_{1:n}, p) \mid X_{1:n} = x_{1:n}}$ is differentiable \wrt{} p.  Define $g: [-1, +1] \to \reals$ by
    \begin{align}
        g(p) = \ex{\tilde{f}(X_{1:n}, p)},
    \end{align}
    where the expectation is taken over $X_{1:n} \sim \pmBernoulli{p}^{n}$ as well as the stochasticity of $\tilde{f}$.
    Then
    \begin{align}
        \ex{\tilde{f}(X_{1:n}) \cdot \sum_{i=1}^n (X_i - p)} = (1-p^2) \cdot \left(g'(p) - \ex[X_{1:n} \sim \pmBernoulli{p}^n]{\diff{\ex{\tilde{f}(X_{1:n}, p) \mid X_{1:n}}}{p}}\right).
    \end{align}
    % where $\one$ is the $d$-dimensional all-one vector, and the column vector $\jacobian{g}(p) \defeq \begin{bmatrix} g_1'(p), \dots, g_d'(p) \end{bmatrix}^\top$ is the Jacobian of $g$ at $p$.
\end{lemma}
\begin{proof}
    % Compared to the original version, this lemma extends on dimensionality and stochasticity of $f$. 
    % Therefore, the proof first assume a deterministic $f$ to extends the dimensionality and then extends on the stochasticity.

    % Firstly, assume $f$ is deterministic. 
    % \begin{align}
        % \ex{\sum_{i=1}^n (X_i - p \cdot \one)^\top f(X_{1:n})}
        % =&  \sum_{j=1}^d \ex{\sum_{i=1}^n (X_{i, j} - p) \cdot f_j(X_{1:n})}\\
        % =&  \sum_{j=1}^d \ex[X_{1:n, -j}]{\ex[X_{1:n, j}]{\sum_{i=1}^n (X_{i, j} - p) \cdot f_j(X_{1:n}) \mid X_{1:n, -j}}}
    % \end{align}

    % Fix a $j$ and $x_{1:n, -j}$. Then $f_j(X_{1:n})$ becomes a deterministic function of $X_{1:n, j}$. Applying the original lemma \citet{bun_make_2017}, we have
    % \begin{align}
        % \ex[X_{1:n, j}]{\sum_{i=1}^n (X_{i, j} - p) \cdot f_j(X_{1:n}) \mid x_{1:n, -j}} = (1-p^2) \cdot g_j'(p \mid x_{1:n, -j}),
    % \end{align}
    % where 
    % \begin{align}
        % g_j(p \mid x_{1:n, -j}) 
        % \defeq& \ex[X_{1:n, j} \sim \pmBernoulli{p}^{n}]{f_j (X_{1:n}) \mid x_{1:n, -j}}
        % =  \sum_{x_{1:n, j}} f_j (x_{1:n}) p(X_{1:n, j}).
    % \end{align}
    % Taking expectations over $X_{1:n, -j}$ leads to
    % \begin{align}
        % \ex[X_{1:n, j}]{g'} = (1-p^2) \cdot g_j'(p \mid x_{1:n, -j})
    % \end{align}
    
    % Plugging this back, we can finish the dimensionality part: 
    % \begin{align}
        % \ex{\sum_{i=1}^n (X_i - p \cdot \one)^\top f(X_{1:n})}
        % =&  \sum_{j=1}^d \ex[X_{1:n, -j}]{(1-p^2) \cdot g_j'(p)}
    % \end{align}

    According to the proof of Lemma A.1 of \citet{bun_make_2017}, for any $x_{1:n}$ and $p$, we have
    \begin{align}
        \frac{\dd \probability{x_{1:n} \mid p}}{\dd p} = \probability{x_{1:n} \mid p} \sum_{i=1}^n \frac{x_i - p}{1 - p^2}. 
    \end{align}

    Firstly, assume $f$ is deterministic. Then 
    \begin{align}
        g'(p) 
        =&  \frac{\dd}{\dd p} \sum_{x_{1:n}} f(x_{1:n}, p) \cdot \probability{x_{1:n} \mid p}\\
        =& \sum_{x_{1:n}} \diff{f(x_{1:n}, p)}{p} \cdot \probability{x_{1:n} \mid p} + \sum_{x_{1:n}} f(x_{1:n}, p) \frac{\dd \probability{x_{1:n} \mid p}}{\dd p}\\
        =& \sum_{x_{1:n}} \diff{f(x_{1:n}, p)}{p} \cdot \probability{x_{1:n} \mid p} + \sum_{x_{1:n}} f(x_{1:n}, p) \cdot \probability{x_{1:n} \mid p} \sum_{i=1}^n \frac{x_i - p}{1 - p^2}\\
        =& \sum_{x_{1:n}} \diff{f(x_{1:n}, p)}{p} \cdot \probability{x_{1:n} \mid p} + \ex{f(X_{1:n}, p) \cdot  \sum_{i=1}^n \frac{X_i - p}{1-p^2}}.
    \end{align}

    We focus on the first term and taking expectation over $p$:
    \begin{align}
        &       \int_{-1/3}^{1/3} (1/9 - p^2) \sum_{x_{1:n}} \diff{f(x_{1:n}, p)}{p} \cdot \probability{x_{1:n} \mid p} \dd p\\
        =&      \sum_{x_{1:n}} \left(\int_{-1/3}^{1/3} (1/9 - p^2) \diff{f(x_{1:n}, p)}{p} \cdot \frac{\density{p \mid x_{1:n}} \cdot \probability{x_{1:n}}}{\density{p}} \dd p\right)\\
        =&      \sum_{x_{1:n}} \probability{x_{1:n}} \left(\int_{-1/3}^{1/3} (1/9 - p^2) \diff{f(x_{1:n}, p)}{p} \cdot \frac{\density{p \mid x_{1:n}}}{\density{p}} \dd p\right)\\
        =&      \sum_{x_{1:n}} \frac{\probability{x_{1:n}}}{3/2} \left(\int_{-1/3}^{1/3} (1/9 - p^2) \diff{f(x_{1:n}, p)}{p} \cdot \density{p \mid x_{1:n}} \dd p\right)\\
    \end{align}

    Taking expectation over $p$ leads to 
    \begin{align}
        & \ex{(1/9-P^2) g'(P)}\\
        =&  \ex{\frac{1/9 - P^2}{1-P^2} f(X_{1:n}, P) \sum_{i=1}^n (X_i - P)} + \int_{-1/3}^{1/3} (1/9 - p^2) \sum_{x_{1:n}} \diff{f(x_{1:n}, p)}{p} \probability{x_{1:n} \mid p} \dd p\\
        =&  \ex{\frac{1/9 - P^2}{1-P^2} f(X_{1:n}, P) \sum_{i=1}^n (X_i - P)} + \sum_{x_{1:n}} \int_{-1/3}^{1/3} (1/9 - p^2) \probability{x_{1:n} \mid p} \diff{f(x_{1:n}, p)}{p} \dd p.
    \end{align}
    By integral by part, we have
    \begin{align}
        & \sum_{x_{1:n}} \int_{-1/3}^{1/3} (1/9 - p^2) \probability{x_{1:n} \mid p} \diff{f(x_{1:n}, p)}{p} \dd p\\
        =&  \sum_{x_{1:n}} \left(
                ((1/9 - p^2) f(x_{1:n}, p) \probability{x_{1:n} \mid p}) \mid^{1/3}_{-1/3} - \int_{-1/3}^{1/3} f(x_{1:n}, p) \dd ((1/9 - p^2) \probability{x_{1:n} \mid p})
            \right)\\
        =&  - \sum_{x_{1:n}}  \int_{-1/3}^{1/3} f(x_{1:n}, p) ((1/9-p^2)\probability{x_{1:n} \mid p} \sum_{i=1}^n \frac{x_i - p}{1 - p^2} + (-2p) \probability{x_{1:n} \mid p}) \dd p \\
        =&  - \ex{\frac{1/9 - P^2}{1-P^2} f(X_{1:n}, P) \sum_{i=1}^n (X_i - P)} + 2 \ex{f(X_{1:n}, P) \cdot P}.
    \end{align} 

    Define deterministic mapping $F: \set{\pm 1}^n \to \reals$ by
    \begin{align}
        F(x_{1:n}) \defeq \ex{f(x_{1:n})}.
    \end{align}
    Then we have
    \begin{align}
        g(p) 
        \defeq \ex{f(X_{1:n})} 
        = \ex[X_{1:n} \sim \pmBernoulli{p}^n]{\ex{f(X_{1:n}) \mid X_{1:n}}} = \ex{F(X_{1:n})}.
    \end{align}
    The original lemma of \citet{bun_make_2017} can be applied to the deterministic $F$ and gives
    \begin{align}
        &g'(p) (1-p^2)\\
        =& \ex[X_{1:n}]{F(X_{1:n}) \cdot \sum_{i=1}^n (X_i - p)}
        = \ex[X_{1:n}]{\ex{f(X_{1:n}) \mid X_{1:n}} \cdot \sum_{i=1}^n (X_i - p)}\\
        =& \ex[X_{1:n}]{\ex{f(X_{1:n}) \cdot \sum_{i=1}^n (X_i - p) \mid X_{1:n}}}
        = \ex{f(X_{1:n}) \cdot \sum_{i=1}^n (X_i - p)}.
    \end{align}

\end{proof}

\NewDocumentCommand{\uniform}{m}{U[#1]}
For a bounded interval $[a, b]$, let $\uniform{a, b}$ denotes the uniform distribution over it. Replacing \citet{bun_make_2017}'s Lemma A.1 with \cref{lemma:expectation_and_derivative}, one can prove the following corollary:
\NewDocumentCommand{\convenientUniform}{}{\uniform{-\frac{1}{3}, +\frac{1}{3}}}
\begin{corollary}[Extended from Lemma 54 of \citet{kamath_privately_2019}]\label{lemma:fingerprinting}
    Let $f$ be a \emph{stochastic} mapping from $\set{-1, +1}^n$ to $[-1/3, +1/3]$. Then we have
    \begin{align}
        \ex[P\sim \convenientUniform, X_{1:n} \sim \pmBernoulli{P}^n]{(f(X_{1:n}) - P)^2 + \left(\frac{\frac{1}{9} - P^2}{1-P^2}\right) \cdot (f(X_{1:n}) - P) \cdot \sum_{i=1}^n(X_i - P)} \ge \frac{1}{27}.
    \end{align}
\end{corollary}

\begin{proof}
    
\end{proof}


\begin{proof}[\cref{prop:minimax_negative}]
The construction of failure and the proof follow \citet{livni2024information}. However, we use the squared difference term of \cref{lemma:fingerprinting} in a different way to cover the distortion term in the rate-distortion bound.

\subsubsection{Construction}

For any sample number $n \in \nats^+$, let the dimension $d \defeq$
\TODO{}.
Then let $\samples \defeq \set{-1, +1}^d$ and $\weights \defeq \set{x \in \reals^d: \norm{x} <= 1}$. Let the loss be $\sampleLoss: \weights \times \samples \to \reals$ defined as
\begin{align}
    \sampleLoss(w, z) \defeq \norm{w - z}^2.
\end{align}
It can be verified that the hypothesis space is convex and has a diameter $D = 2$. The loss function is also convex and $4$-Lipschitz within $\weights \times \samples$.
Therefore, the 

The construction has several desirable properties. For example, one can access the excess risks using the distances in the parameter space: for any distribution $\mu$ over $\samples$,
\begin{align}
    \poploss[\mu]{w} - \poploss[\mu]{w^*}
    =&  \ex{\norm{w - w^*}^2},
\end{align}
where $w^*$ is the minimizer for $\mu$. See (9) of \citet{livni2024information} for a proof.

\subsubsection{Proof of Failure}

Assume the 

\end{proof}

==> theory/optimization.tex <==
\section{Details in Bound Optimization}\label{appendix:bound_optimization}

As outlined in \cref{sec:flatness_bound}, we first approximate the losses to the second order. Therefore, in the surrogate optimization we have
\begin{align}
    \Delta_{\Delta G}(\weight_T, \trainingSet) \approx& \Delta G^\top \nabla \emploss{\weight_T} + \frac{1}{2} \Delta G^\top \emphessian \Delta G,\\
    \Delta_{\Delta G}(\weight_T, \trainingSet') \approx& \Delta G^\top \nabla \poploss{\weight_T} + \frac{1}{2} \Delta G^\top \pophessian \Delta G,\\
    \Delta^{T \sigma^2}(\weight_T + \Delta G, \trainingSet) \approx& \ex[\epsilon \sim \gaussian[0][T \sigma^2 I]]{\epsilon^\top \nabla \emploss{\weight_T + \Delta G} + \frac{1}{2}\epsilon^\top \emphessian \epsilon} = \frac{\sigma^2 T}{2} \trace{\emphessian},\\
    \Delta^{T \sigma^2}(\weight_T + \Delta G, \trainingSet') \approx& \ex[\epsilon \sim \gaussian[0][T \sigma^2 I]]{\epsilon^\top \nabla \poploss{\weight_T + \Delta G} + \frac{1}{2}\epsilon^\top \pophessian \epsilon} = \frac{\sigma^2 T}{2} \trace{\pophessian}.
\end{align}


